A double integral of dlog forms which is not polylogarithmic

Feynman integrals are central to all calculations in perturbative Quantum Field Theory. They often give rise to iterated integrals of dlog-forms with algebraic arguments, which in many cases can be evaluated in terms of multiple polylogarithms. This has led to certain folklore beliefs in the community stating that all such integrals evaluate to polylogarithms. Here we discuss a concrete example of a double iterated integral of two dlog-forms that evaluates to a period of a cusp form. The motivic versions of these integrals are shown to be algebraically independent from all multiple polylogarithms evaluated at algebraic arguments. From a mathematical perspective, we study a mixed elliptic Hodge structure arising from a simple geometric configuration in $\mathbb{P}^2$, consisting of a modular plane elliptic curve and a set of lines which meet it at torsion points, which may provide an interesting worked example from the point of view of periods, extensions of motives, and L-functions.

==> conventions.tex <==
% !TEX root = main.tex

\section*{CONVENTIONS}

{\bf [THIS SECTION IS ONLY MEANT TO SET THE CONVENTIONS, AND CAN BE REMOVED AT THE END]}

We normalise our integrals such that
\beq
\int_{0\le x_1\le x_2\le1}dx_1\wedge dx_2 =\int_{0}^1dx_2 \left(\int_0^{x_2}dx_1\right)= \frac{1}{2}\,.
\eeq 
Note that with this convention the `order of integration' is reversed with respect to the order in which the variables appear in the wedge product.
\franciscomment{I agree with the formula, but added the brackets to show that the $x_1$ integral is done first in your notation (I would write it a bit differently, but no matter).}
\franciscomment{Actually by Fubini's theorem it doesn't matter in which order the integral is performed. The point is just that the order of the forms in the integrand determines an orientation of the plane, and we agree that the domain of integration is oriented positively with respect to it. Check:
$$\int_{x_1}^1 dx_2 = (1-x_1) $$
$$ \int_{0\leq x_2 \leq 1} dx_1 \left(\int_{x_1}^1 dx_2\right) =  \int_{0\leq x_2 \leq 1} (1-x_1) dx_1 = 1-1/2 = 1/2$$
}

Our definition of iterated integrals is (notations are as in Section~\ref{sec:introduction}):
\beq\bsp
\int_{\gamma}&\,\omega_1\cdots\omega_n :=\int_{0\le t_1\le t_2\le \cdots\le t_n\le 1}\gamma^{\ast}\omega_1\wedge\ldots\wedge \gamma^{\ast}\omega_n\\
&= \int_{0\le t_1\le t_2\le \cdots\le t_n\le 1}dt_1\,f_1(t_1)\cdots dt_n\,f_n(t_n)\\
&=\int_0^1dt_n\,f_n(t_n)\int_0^{t_n}dt_{n-1}\cdots\int_0^{t_2}dt_1\,f_1(t_1)\,.
\esp\eeq
\franciscomment{OK}
\subsection*{The integral $I_{\mathcal{E}}$}

A primitive of the form $\omega$ in~\eqref{omegadef} is
\beq
F = -\omega_x\,\log\frac{y+1}{y-1} = -\frac{2}{3}\,\left(\frac{1+x}{x^2}\right)\,\frac{dy}{y}\,\log\left(\frac{y+1}{y-1}\right)\,,
\eeq
\franciscomment{I agree with this, there was a sign error in the text}
i.e., we have $dF=\omega$. Here we have chosen a branch such that $x=(y^2-1)^{1/3}$. Since $\partial\sigma_\E=\frac{1}{2}(c+\bar{c})$, Stokes' theorem implies
\beq
I_\E = \int_{\sigma_{\E}}\pi^*(\omega) = \int_{\sigma_\E}dF = \int_{\frac{1}{2}(c+\bar{c})}F\big|_{\E} = \textrm{Re}\int_cF\big|_{\E}
=-\frac{2}{3}\,\textrm{Re}\int_{-\infty}^{\infty}\frac{dy}{y}\,\left(\frac{1+x}{x^2}\right)\,\log\left(\frac{y+1}{y-1}\right)\,.
\eeq
The integrand is invariant under $y\leftrightarrow -y$, and so we can write
\beq
I_\E = -\frac{4}{3}\,\textrm{Re}\int_{0}^{\infty}\frac{dy}{y}\,\left(\frac{1+x}{x^2}\right)\,\log\left(\frac{y+1}{y-1}\right)\,.
\eeq
We now change variables via $y=\sqrt{1+x^3}$. We find
\beq\bsp\label{conv:I_E_1}
I_\E &\,= -2\,\textrm{Re}\int_{-1}^{\infty}\frac{dx}{x^2-x+1}\,\log\left(\frac{\sqrt{1+x^3}+1}{\sqrt{1+x^3}-1}\right)\\
&\,= -2\,\textrm{Re}\int_{-1}^{\infty}\frac{dx_1}{x_1^2-x_1+1}\,\int_{-1}^{x_1}d\log\left(\frac{\sqrt{1+x_2^3}+1}{\sqrt{1+x_2^3}-1}\right)\\
&\,= -2\,\textrm{Re}\int_{-1}^{\infty}\frac{1}{\rho-\bar{\rho}}\,d\log\left(\frac{x_1-\rho}{x_1-\bar{\rho}}\right)\,\int_{-1}^{x_1}d\log\left(\frac{\sqrt{1+x_2^3}+1}{\sqrt{1+x_2^3}-1}\right)\\
&\,=-2\textrm{Re}\int_{-1\le x_2\le x_1\le \infty}\frac{1}{\rho-\bar{\rho}}\,d\log\left(\frac{\sqrt{1+x_2^3}+1}{\sqrt{1+x_2^3}-1}\right)\wedge d\log\left(\frac{x_1-\rho}{x_1-\bar{\rho}}\right)\\
&\,=+2\,\textrm{Re}\int_{-1\le x_2\le x_1\le \infty} \frac{1}{\rho-\bar{\rho}}\,d\log\left(\frac{x_1-\rho}{x_1-\bar{\rho}}\right)\wedge d\log\left(\frac{\sqrt{1+x_2^3}+1}{\sqrt{1+x_2^3}-1}\right)
\,.
\esp\eeq
Note the sign change in the last step!
%\franciscomment{ There is an issue here: the factor $\frac{2}{\rho - \overline{\rho}}$ is not real so one can't pull it out of the real part}
\franciscomment{  I was writing it differently:  
Note that
 $$\int_{x_1}^{\infty}   d\log\left(\frac{\sqrt{1+x_2^3}+1}{\sqrt{1+x_2^3}-1}\right) = - d\log\left(\frac{\sqrt{1+x_1^3}+1}{\sqrt{1+x_1^3}-1}\right)$$
so we  get
$$I_{\mathcal{E}}= \textrm{Re}  \int_{-1\le x_1\le x_2\le \infty} \frac{dx}{x^2-x+1} \wedge d\log\left(\frac{\sqrt{1+x_2^3}+1}{\sqrt{1+x_2^3}-1}\right)  $$
or
$$I_{\mathcal{E}}= \textrm{Re} \, \frac{2}{\rho-\bar{\rho}}\int_{-1\le x_1\le x_2\le \infty} d\log\left(\frac{x_1-\rho}{x_1-\bar{\rho}}\right) \wedge d\log\left(\frac{\sqrt{1+x_2^3}+1}{\sqrt{1+x_2^3}-1}\right)  $$
I prefer this way of writing it because it is exactly parallel with the case of $I$ below, and also is on the nose an iterated integral between cusps on the modular curve.
}
\claudecomment{Yes, I agree with this, and I also like this way of writing the integrals better!}

In order to evaluate this integral, we start from the first line in~\eqref{conv:I_E_1} and write it as:
\beq\bsp
I_\E &\, = -2\,\textrm{Re}\left[\int_{-1}^{0}\frac{dx}{x^2-x+1}\,\log\left(\frac{\sqrt{1+x^3}+1}{\sqrt{1+x^3}-1}\right)+\int_{0}^{\infty}\frac{dx}{x^2-x+1}\,\log\left(\frac{\sqrt{1+x^3}+1}{\sqrt{1+x^3}-1}\right)\right]\,.
\esp\eeq
In the first term we have ${\sqrt{1+x^3}-1}\le 0$, and so, for some choice of branch of log, 
\beq
\log\left(\frac{\sqrt{1+x^3}+1}{\sqrt{1+x^3}-1}\right) = \log\left(\frac{1+\sqrt{1+x^3}}{1-\sqrt{1+x^3}}\right) + i\pi\,,\qquad \textrm{for } -1<x<0\,.
\eeq
We can however drop the imaginary part, since we are only interested in the real part of the integral. We can then drop the Re-operation all together, and we have
 \beq\bsp
I_\E &\, = -2\,\left[\int_{-1}^{0}\frac{dx}{x^2-x+1}\,\log\left(\frac{1+\sqrt{1+x^3}}{1-\sqrt{1+x^3}}\right)+\int_{0}^{\infty}\frac{dx}{x^2-x+1}\,\log\left(\frac{\sqrt{1+x^3}+1}{\sqrt{1+x^3}-1}\right)\right]\,.
\esp\eeq
We can evaluate these two integrals numerically with high precision (simply using {\tt NIntegrate} in {\sc Mathematica}). We find
\beq
I_\E = -18.6572279896368252\ldots = -4\pi\sqrt{3}\,\Lambda(f,2)\,.
\eeq
\franciscomment{I agree that the integral is negative, now} 


\subsection*{The integral $I$}
From~\eqref{eq:I_def_2}:
\beq\bsp\label{conv:I_int}
I &\,= \frac{1}{\rho-\bar{\rho}}\int_{2\le x_1\le x_2\le\infty}d\log\left(\frac{x_1-\rho}{x_1-\bar{\rho}}\right)\wedge d\log\left(\frac{\sqrt{1+x_2^3}+1}{\sqrt{1+x_2^3}-1}\right)\\
&\,= \frac{1}{\rho-\bar{\rho}}\int_{2}^{\infty} d\log\left(\frac{\sqrt{1+x_2^3}+1}{\sqrt{1+x_2^3}-1}\right)\int_2^{x_2}d\log\left(\frac{x_1-\rho}{x_1-\bar{\rho}}\right)\\
&\,= \frac{1}{\rho-\bar{\rho}}\int_{2}^{\infty} dx_2\,\left(\partial_{x_2}\log\left(\frac{\sqrt{1+x_2^3}+1}{\sqrt{1+x_2^3}-1}\right)\right)\,\left[\log\left(\frac{x_2-\rho}{x_2-\bar{\rho}}\right)-\log\left(\frac{2-\rho}{2-\bar{\rho}}\right)\right]\,.
\esp\eeq
The last integral can be evaluated numerically to high precision:
\beq\bsp
I&\,=-0.179654\ldots\\
&\,=-\frac{2\pi}{\sqrt{3}}\,\Lambda(f,2)+\frac{5}{\sqrt{3}}\,\textrm{Cl}_2\left(\frac{\pi}{3}\right)\\
&\,=\frac{1}{6}\,I_{\E}+\frac{5}{\sqrt{3}}\,\textrm{Cl}_2\left(\frac{\pi}{3}\right)\,.
\esp\eeq
%\franciscomment{I think you mean $I$ in the first line here}
\franciscomment{I agree that this integral is negative: it is 
$$
I = \int_{2\le x_1\le x_2\le\infty} \frac{dx_1}{x_1^2-x_1+1} \wedge d\log\left(\frac{\sqrt{1+x_2^3}+1}{\sqrt{1+x_2^3}-1}\right)$$
$$
 -  \int_{2\le x_1\le\infty} \frac{dx_1}{x_1^2-x_1+1} \wedge \log\left(\frac{\sqrt{1+x_1^3}+1}{\sqrt{1+x_1^3}-1}\right)$$
so is negative for the same reasons as the previous integral. 
}


We can write the $d\log$-forms as Eisenstein series, see~\eqref{eq:dlog_to_eisenstein}. We have $x_6(0) = 2$ and $x_6(i\infty) = \infty$. Hence, starting from the first line of~\eqref{conv:I_int}, and changing variables to $(x_1,x_2) = (x_6(it_1),x_6(it_2))$,
\beq\bsp
I &\,= \frac{1}{\rho-\bar{\rho}}\int_{0\le t_1\le t_2\le\infty}\frac{dt_1\wedge dt_2}{(2\pi)^2}\,E_1(it_1)\,E_2(it_2)\\
&\,= \frac{1}{(2\pi)^2(\rho-\bar{\rho})}\int_{0}^{\infty}dt_2\,E_2(it_2)\,\int_0^{t_2}dt_1\,E_1(it_1)\\
&\,= \frac{1}{(2\pi)^2(\rho-\bar{\rho})}\int_{\infty}^{0}dt_1\,E_1(it_1)\,\int_\infty^{t_1}dt_2\,E_2(it_2)\,.
\esp\eeq
I can evaluate the last version of the integral numerically with my code, and it agrees with the value quoted before.




